Recursive Backwards Q-Learning in Deterministic Environments

Reinforcement learning is a popular method of finding optimal solutions to complex problems. Algorithms like Q-learning excel at learning to solve stochastic problems without a model of their environment. However, they take longer to solve deterministic problems than is necessary. Q-learning can be improved to better solve deterministic problems by introducing such a model-based approach. This paper introduces the recursive backwards Q-learning (RBQL) agent, which explores and builds a model of the environment. After reaching a terminal state, it recursively propagates its value backwards through this model. This lets each state be evaluated to its optimal value without a lengthy learning process. In the example of finding the shortest path through a maze, this agent greatly outperforms a regular Q-learning agent.

==> diagramme/arrows/down.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,-1);
\end{tikzpicture}

==> diagramme/arrows/downleft.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,-1);
    \draw[-{latex}] (0,0) to (-1,0);
\end{tikzpicture}

==> diagramme/arrows/downleftright.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,-1);
    \draw[-{latex}] (0,0) to (-.75,0);
    \draw[-{latex}] (0,0) to (.75,0);
\end{tikzpicture}

==> diagramme/arrows/downright.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,-1);
    \draw[-{latex}] (0,0) to (1,0);
\end{tikzpicture}

==> diagramme/arrows/left.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (-1,0);
\end{tikzpicture}

==> diagramme/arrows/leftright.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (-.75,0);
    \draw[-{latex}] (0,0) to (.75,0);
\end{tikzpicture}

==> diagramme/arrows/leftupdown.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,.75);
    \draw[-{latex}] (0,0) to (0,-.75);
    \draw[-{latex}] (0,0) to (-1,0);
\end{tikzpicture}

==> diagramme/arrows/omni.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,0.75);
    \draw[-{latex}] (0,0) to (0,-0.75);
    \draw[-{latex}] (0,0) to (0.75,0);
    \draw[-{latex}] (0,0) to (-0.75,0);
\end{tikzpicture}

==> diagramme/arrows/right.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (1,0);
\end{tikzpicture}

==> diagramme/arrows/rightupdown.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,.75);
    \draw[-{latex}] (0,0) to (0,-.75);
    \draw[-{latex}] (0,0) to (1,0);
\end{tikzpicture}

==> diagramme/arrows/up.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,1);
\end{tikzpicture}

==> diagramme/arrows/updown.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,.75);
    \draw[-{latex}] (0,0) to (0,-.75);
\end{tikzpicture}

==> diagramme/arrows/upleft.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,1);
    \draw[-{latex}] (0,0) to (-1,0);
\end{tikzpicture}

==> diagramme/arrows/upleftright.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,1);
    \draw[-{latex}] (0,0) to (-.75,);
    \draw[-{latex}] (0,0) to (-.75,0);
\end{tikzpicture}

==> diagramme/arrows/upright.tex <==
\begin{tikzpicture}[scale=0.325]
    \draw[-{latex}] (0,0) to (0,1);
    \draw[-{latex}] (0,0) to (1,0);
\end{tikzpicture}
